DrugOOD: Out-of-Distribution (OOD) Dataset Curator and Benchmark for AI-aided Drug Discovery -- A Focus on Affinity Prediction Problems with Noise Annotations

AI-aided drug discovery (AIDD) is gaining increasing popularity due to its promise of making the search for new pharmaceuticals quicker, cheaper and more efficient. In spite of its extensive use in many fields, such as ADMET prediction, virtual screening, protein folding and generative chemistry, little has been explored in terms of the out-of-distribution (OOD) learning problem with \emph{noise}, which is inevitable in real world AIDD applications. In this work, we present DrugOOD, a systematic OOD dataset curator and benchmark for AI-aided drug discovery, which comes with an open-source Python package that fully automates the data curation and OOD benchmarking processes. We focus on one of the most crucial problems in AIDD: drug target binding affinity prediction, which involves both macromolecule (protein target) and small-molecule (drug compound). In contrast to only providing fixed datasets, DrugOOD offers automated dataset curator with user-friendly customization scripts, rich domain annotations aligned with biochemistry knowledge, realistic noise annotations and rigorous benchmarking of state-of-the-art OOD algorithms. Since the molecular data is often modeled as irregular graphs using graph neural network (GNN) backbones, DrugOOD also serves as a valuable testbed for \emph{graph OOD learning} problems. Extensive empirical studies have shown a significant performance gap between in-distribution and out-of-distribution experiments, which highlights the need to develop better schemes that can allow for OOD generalization under noise for AIDD.

==> def_global.tex <==
%\newcommand{\srcpath}{srcs/}
%\newcommand{\utilspath}{../utils/}
\usepackage{jmlr2e_cus}
\usepackage[usenames]{xcolor}
%\usepackage[usenames]{color}
\usepackage[bookmarksnumbered=true]{hyperref}
\usepackage{url}
%\definecolor{cite_color}{RGB}{0, 51, 153}
% \definecolor{cite_color}{RGB}{0, 0, 255}
\definecolor{cite_color}{HTML}{114083}
%\definecolor{link_color}{RGB}{0,102,102}%  green-style
\definecolor{link_color}{RGB}{153, 0,0}  %  red
\definecolor{url_color}{RGB}{153, 102,  0}
\definecolor{emp_color}{RGB}{0,0,255}
% {51, 102, 51}
\hypersetup{
 colorlinks,
 citecolor=cite_color,
 linkcolor=link_color,
 urlcolor=url_color}
 % graph
\graphicspath{{./figs/}}

\usepackage{framed}
\definecolor{shadecolor}{rgb}{0.94, 0.97, 1.0}
% \definecolor{beaublue}{rgb}{0.74, 0.83, 0.9}

\usepackage{epsfig}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{graphicx}
\usepackage{subfig}
\usepackage{multirow}
\usepackage{booktabs}
%\usepackage{mathrsfs}
\usepackage{wrapfig}
\usepackage{tikz,siunitx,mwe}
\usepackage{caption}
\usepackage{enumerate}
\usepackage{bm}
%\usepackage{bbm}
% to use \bm in section title
\pdfstringdefDisableCommands{%
	\renewcommand*{\bm}[1]{#1}%
	% any other necessary redefinitions
}
\usepackage{tabularx}

% citation
%\usepackage[]{biblatex}
\usepackage{natbib}
\bibpunct{(}{)}{;}{a}{,}{,}
%1 the opening bracket symbol, default = (
%2 the closing bracket symbol, default = )
%3 the punctuation between multiple citations, default = ;
%4 the letter `n’ for numerical style, or `s’ for numerical superscript style, any other letter for author-year, default = author-year;
%5 the punctuation that comes between the author names and the year
%6 the punctuation that comes between years or numbers when common author lists are suppressed (default = ,);
\bibliographystyle{icml2017}
%  abbrvnat  plainnat icml2017


\usepackage{mathtools}


% For algorithms, use algorithm2e
\usepackage[vlined, ruled, linesnumbered]{algorithm2e}
%set comment style
\newcommand\mycommfont[1]{\footnotesize\textit{
\hspace{-.3em}#1}}
\SetCommentSty{mycommfont}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}

 \usepackage{cleveref} % should be put after other packages
 %  using always captial letter
 \crefname{section}{Section}{Sections}
 \crefname{theorem}{Theorem}{Theorems}
 \crefname{lemma}{Lemma}{Lemmas}
 \crefname{equation}{Equation}{Equations}
 \crefname{proposition}{Proposition}{Propositions}
 \crefname{claim}{Claim}{Claims}
\crefname{appendix}{Appendix}{Appendices}
   \crefname{algorithm}{Algorithm}{Algorithms}
 \crefname{figure}{Figure}{Figures}
 \crefname{table}{Table}{Tables}
 \crefname{remark}{Remark}{Remarks}
 \crefname{definition}{Definition}{Definitions}
 \crefname{equatinon}{Equation}{Equations}
 \crefname{corollary}{Corollary}{Corollaries}
 %  \crefname{equation}{Equation}{Equations}
 %  \crefname{proposition}{proposition}{propositions}
 %  \crefname{claim}{claim}{claims}
 % usage:
 %In the first argument of \crefname{}{}{} comes the type of reference (equation, figure, table, section, etc.). The second argument contains the word that is printed if only one reference is made and the third argument contains the plural form for multiple references.


\allowdisplaybreaks

\usepackage{thmtools}
\usepackage{thm-restate}
%one example:
%\begin{theorem}[name=good,restate=foo]
%content...
%\end{theorem}
%\foo*


%  circled text
%\textcircled{\raisebox{-0.9pt}{8}}
\let \oldtextcircled \textcircled
\renewcommand{\textcircled}[1]{\oldtextcircled{\footnotesize #1}}

% visual
\newcommand{\scalebarimg}[3]{
  \begin{tikzpicture}
    \draw node[name=micrograph] {\includegraphics[width=#2\textwidth]{#1}}; %I fetch the image %I draw the scalebar
    \draw  (micrograph.north west)  node[anchor=north west,yshift=-1, ]{\textbf{\small{#3}}}; %I draw the image label
  \end{tikzpicture}
}


\def\labelitemi{-}
% set margin of list
\usepackage{enumitem}
\setlist[itemize]{leftmargin=9mm}


\newcommand{\todo}[1]{\textcolor{blue}{TODO:#1}}
%\usepackage[textsize=small]{todonotes}
\newcommand{\appendixtitle}[1]{
	\begin{center}
		\LARGE \bf #1
	\end{center}
}

% statistical notations

% independent 
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}


\def\C{{\cal C}}
\def\S{{\cal S}}
\def\E{{\mathbb E}}
\def\X{{\cal X}}
\def\Y{{\cal Y}}
\def\H{{\mathbb  H}}
\def\Z{{\mathbb Z}}
\def\L{{\cal L}}
\def\N{{\cal N}}

\def\cone{{\cal K}}

%\def\A{{\mathscr A}}
\def\M{{\cal M}}
\def \I {{\cal{I}}}
\def\T {\mathbb{T}}
\def\opt{\ensuremath{\Omega^*}}
\def\optcont{\ensuremath{\x^*}}
\newcommand{\opti}[1]{x^*_{#1}} % ith entry of opt, used
% in double greedy proof

%% bold small letters
%\def \c{\bm{c}}
%\def \v{\bm{v}}
%\def \w{\bm{w}}
%\def \r{\bm{r}}
%\def \b{\bm{b}}
%\def \d{\bm{d}}
%\def \a{\bm{a}}
%\def \x{\mathbf{x}}
%\def \y{\bm{y}}
%\def \s{\bm{s}}
%\def \e{\bm{e}}
%\def \u{\bm{u}}
%\def \bmu{\bm{u}}
%\def \z{\bm{z}}
%\def \h{\bm{h}}



% bold small letters
\def \c{\mathbf{c}}
\def \v{\mathbf{v}}
\def \w{\mathbf{w}}
\def \r{\mathbf{r}}
\def \a{\mathbf{a}}
\def \b{\mathbf{b}}
\def \d{\mathbf{d}}
\def \x{\mathbf{x}}
\def \y{\mathbf{y}}
\def \s{\mathbf{s}}
\def \e{\mathbf{e}}
\def \u{\mathbf{u}}
\def \bmu{\mathbf{u}}
\def \t{\mathbf{t}}
\def \z{\mathbf{z}}
\def \h{\mathbf{h}}
\def \bu{\mathbf{u}}


\def \BA{\mathbf{A}}
\def \BB{\mathbf{B}}
\def \BX{\mathbf{X}}
\def \BY{\mathbf{Y}}
\def \BI{\mathbf{I}}
\def \BC{\mathbf{C}}
\def \BD{\mathbf{D}}
\def \BE{\mathbf{E}}
\def \BH{\mathbf{H}}
\def \BL{\mathbf{L}}
\def \BM{\mathbf{M}}
\def \BG{\mathbf{G}}
\def \BP{\mathbf{P}}
\def \BQ{\mathbf{Q}}
\def \BR{\mathbf{R}}
\def \BS{\mathbf{S}}
\def \BU{\mathbf{U}}
\def \BV{\mathbf{V}}
\def \BW{\mathbf{W}}
\def \BZ{\mathbf{Z}}
% compatibable with aistats
\def \bmA{\mathbf{A}}
\def \bmH{\mathbf{H}}
\def \bmL{\mathbf{L}}
\def \bmX{\mathbf{X}}
\def \bmY{\mathbf{Y}}
\def \bmI{\mathbf{I}}
\def \bmW{\mathbf{W}}
\def \bmZ{\mathbf{Z}}


\def \BLambda{\mathbf{\Lambda}}  % B or b, depend on the first letter of the symbol
\def \BSigma{\mathbf{\Sigma}}
\def \bsigma{\bm{\sigma}}
\def \btheta{\bm{\theta}}
\def \blambda{\bm{\lambda}}
\def \balpha{\bm\alpha}
\def \bphi{\bm{\phi}}


\def \bmsigma{\bm{\sigma}}
\def \bmtheta{\bm{\theta}}
\def \bmlambda{\bm{\lambda}}
\def \bmalpha{\bm\alpha}
\def \bmphi{\bm{\phi}}
\def \bmchi{\bm{\chi}}


\def \P{{\cal{P}}}
\def \Q{{\cal{Q}}}
\def \W{{\cal{W}}}
\def \B{{\cal{B}}}
\def \R{{\mathbb{R}}}
%  the transpose
\def \trans{\top}
% trace
\newcommand{\tr}[1]{\text{tr}(#1)}
\newcommand{\pare}[1]{{#1}}  % parethese sth, with extra {} added, used in a
% math mode


\def \D{{\cal{D}}}
\def \V{{\cal{V}}}
\def \E{{\mathbb{E}}} %  expection

\newcommand{\MAXCUT}{{\textsc{MaxCut}}}
\newcommand{\LOVASZ}{Lov{\'a}sz }
\newcommand{\maxcut}{{\textsc{MaxCut}}}

\newcommand{\argmin}{{\arg\min}}
\newcommand{\diag}{{\text{diag}}}
\newcommand{\dom}[1]{{\texttt{dom}(#1)}}
\newcommand{\sign}[1]{{\text{sign}(#1)}}
\newcommand{\dep}{{\text{Dep}}} % dependency set of a set function
\newcommand{\var}{{\text{Var}}} %  variance
\newcommand{\argmax}{{\arg\max}}
\newcommand{\algname}[1]{{\textsc{#1}}}
\newcommand{\note}[1]{\textcolor{blue}{//}#1}
%\newcommand{\spt}[1]{{\texttt{supp}^+}(#1)}
\newcommand{\spt}[1]{{\texttt{supp}}(#1)}
\newcommand{\dtp}[2]{\langle #1, #2\rangle}% dot product
\newcommand{\de}[1]{\text{det}\left(#1\right)}% determinant of a square matrix
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\fracppartial}[2]{\frac{\partial^2 #1}{\partial #2}}


\newcommand{\lleq}{\preceq}
\newcommand{\ggeq}{\succeq}
\renewcommand{\ll}{\prec}
\renewcommand{\gg}{\succ}
\newcommand{\leqco}{\leq}

\newcommand{\bas}{\mathbf{e}} % standard basis
%\def \chara{\bm{\chi}} % characteristic vector
\def \chara{\mathbf{e}} % characteristic vector

\def \cg{L}
\def\A{{\mathscr{A}}}

%% Standard
\newcommand{\groundset}{\ensuremath{\mathcal{V}}}
\newcommand{\groundsett}{\ensuremath{{E}}}
\newcommand{\contsub}{continuous submodular }
\newcommand{\NEWDR}{\texttt{weak DR}}


\newcommand{\set}[2]{#1\!\!\gets\!\! #2}
%\newcommand{\sete}[3]{\mathbf #1|#1_{#2}\!\!\gets\!\! #3} 
\newcommand{\sete}[3]{\mathbf #1|_{#2} #3} 
 %  set x(i) to be k,  only make the first argument as bold face, not including the superscript or subscript

% new theorem
%
%\newtheorem{example}{Example}
%\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
%\newtheorem{proposition}{Proposition}[section]
%\newtheorem{remark}{Remark}[section]
%\newtheorem{corollary}{Corollary}[section]
%\newtheorem{definition}{Definition}[section]
%\newtheorem{conjecture}{Conjecture}[section]
%\newtheorem{axiom}{Axiom}[section]
%\newtheorem{claim}{Claim}[section]
\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{claim}{Claim}
\newtheorem{observation}{Observation}


% floor and ceil
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% new
\newcommand{\parti}{\text{Z}} % partition function
\newcommand{\zero}{\mathbf{0}} % vector zero
\newcommand{\one}{\mathbf{1}} % vector zero
\newcommand{\ele}{v} % element of a ground set
\newcommand{\multi}{f_{\text{mt}}} % multilinear extension
\newcommand{\prob}{\text{P}} % probability
\newcommand{\bigo}[1]{\mathcal {O}\! \left(#1\right)}

\newcommand{\EBE}[1]{{\mathbb E}\left[#1\right]}  % expectation with brackets that are extensible
\newcommand{\EB}[1]{{\mathbb E}[#1]}  % expectation with brackets

\newcommand{\mixingmat}{\BW}
\def\dist{{\cal D}} % distribution

\newcommand{\pa}{\text{PA}}
\newcommand{\intermed}{\mathbf{o}}
\def \bu{\mathbf{u}}
\def \bmmu{\bm{\mu}}
\def \m{\mathbf{m}}

\def \flweights {R} % facility location weights


% quantum computing
% Dirac Kets
\newcommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}

% macros from cocoa and cola
\newcommand{\cocoa}{\textsc{CoCoA}\xspace} 
\newcommand{\cola}{\textsc{CoLa}\xspace}
\newcommand{\diging}{{DIGing}\xspace}
\newcommand{\cocoap}{\textsc{CoCoA$\!^{\bf \textbf{\footnotesize+}}$}\xspace}
\newcommand{\cocoapm}{\textsc{CoCoA/$\!^{\bf \textbf{\footnotesize+}}$}\xspace}
\newcommand{\proxcocoa}{\textsc{CoCoA}\xspace}%
\newcommand{\dcocoa}{\textsc{D-CoCoA}\xspace}%
\newcommand{\glmnet}{\textsc{glmnet}\xspace}

% stepsize 
\newcommand{\stepsize}{stepsize\xspace}
\newcommand{\stepsizes}{stepsizes\xspace}


% alg names for cont. submodular max.
\newcommand{\pga}{\algname{PGA}\xspace}
\newcommand{\nonconvexfw}{\algname{non-convex FW}\xspace}
\newcommand{\submodularfw}{\algname{submodular FW}\xspace}
\newcommand{\shrunkenfw}{\algname{shrunken FW}\xspace}
\newcommand{\twophasefw}{\algname{two-phase FW}\xspace}
\newcommand{\ssfw}{\algname{SSFW}\xspace}


% from non-submodular max. 
\def \bmA{\mathbf{A}}
\def \bmB{\mathbf{B}}
\def \bmX{\mathbf{X}}
\def \bmI{\mathbf{I}}
\def \bmC{\mathbf{C}}
\def \bmD{\mathbf{D}}
\def \bmE{\mathbf{E}}
\def \bmL{\mathbf{L}}
\def \bmM{\mathbf{M}}
\def \bmG{\mathbf{G}}
\def \bmP{\mathbf{P}}
\def \bmQ{\mathbf{Q}}
\def \bmLambda{\mathbf{\Lambda}}
\def \bmSigma{\mathbf{\Sigma}}
\def \bmsigma{\bm{\sigma}}
\def \bmtheta{\bm{\theta}}
\def \bmlambda{\bm{\lambda}}
\def \bmalpha{\bm{\alpha}}
\def \bmmu{\bm{\mu}}
\def \bmxi{\bm{\xi}}
% cardinality constraint
\newcommand{\card}{\ensuremath{k}\xspace}

% greedy curvature
\newcommand{\cur}{\ensuremath{\alpha}}
\newcommand{\greedycur}{\ensuremath{\alpha^{\text{G}}}}

% my emph
\newcommand{\emp}[1]{\texttt{#1}}


\newcommand{\shapley}{\ensuremath{\text {Sh}}}
\newcommand{\banzhaf}{\ensuremath{\text {Ba}}}
\newcommand{\lovasz}{f_{\text{lo}}} %  extension
\newcommand{\sigmoid}[1]{\text{sigmoid}(#1)} %  extension


\renewcommand{\mid}{|}
\newcommand{\kl}[2]{\mathbb{KL}(#1\|#2)}
\newcommand{\entropy}[1]{\mathbb{H}(#1)}



